A 1D fluid model of the Centaurus A jet

We implement a steady, one-dimensional flow model for the X-ray jet of Centaurus A in which entrainment of stellar mass loss is the primary cause of dissipation. Using over 260 ks of new and archival Chandra/ACIS data, we have constrained the temperature, density and pressure distributions of gas in the central regions of the host galaxy of Centaurus A, and so the pressure throughout the length of its jet. The model is constrained by the observed profiles of pressure and jet width, and conserves matter and energy, enabling us to estimate jet velocities, and hence all the other flow properties. Invoking realistic stellar populations within the jet, we find that the increase in its momentum flux exceeds the net pressure force on the jet unless only about one half of the total stellar mass loss is entrained. For self-consistent models, the bulk speed only falls modestly, from ~0.67c to ~0.52c over the range of 0.25-5.94 kpc from the nucleus. The sonic Mach number varies between ~5.3 and 3.6 over this range.

==> journals.tex <==
\bibpunct{(}{)}{;}{a}{}{,}
\def\aap{A\&A}                % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}              % Astronomy and Astrophysics, Supplement
\def\aj{AJ}                   % Astronomical Journal
\def\ajph{Australian J.~Phys.}% Australian Journal of Physics
\def\alet{Astro.~Lett.}       % Astronomical Letters
\def\ao{Applied Optics}       % Applied Optics
\def\apj{ApJ}                 % Astrophysical Journal
\def\apjl{ApJ}                % Astrophysical Journal, Letters
\def\apjs{ApJS}              % Astrophysical Journal, Supplement
\def\apss{Ap\&SS}             % Astrophysics and Space Science
\def\araa{ARA\&A}             % Annual Review of Astronomy and Astrophysics
\def\asr{Av.~Space Res.}     % Advances in Space Research
\def\azh{AZh}                 % Astronomiceskij Zhurnal
\def\baas{BAAS}               % Bulletin of the American Astronomical Society
\def\cpc{Comput.~Phys.~Commun.} % Computer Physics Communications
\def\gca{Geochim.~Cosmochim.~Acta} % Cheochimica et Cosmochimica Acta
\def\iaucirc{IAU Circ.}       % International Astronomical Union, Circular
\def\ibvs{IBVS}               % International Bulletin of Variable Stars
\def\icarus{Icarus}           % Icarus
\def\jcomph{J.~Comput.~Phys.} % Journal of Computational Physics
\def\jcp{J.~Chem.~Phys.}      % Journal of Chemical Physics
\def\jgr{J.~Geophys.~R.}      % Journal of Geophysical Research
\def\jrasc{JRASC}             % Journal of the RAS of Canada
\def\met{Meteoritics}         % Meteoritics
\def\mmras{MmRAS}             % Memoirs of the Royal Astronomical Society
\def\mnras{MNRAS}             % Monthly Notices of the RAS
\def\mps{Meteoritics and Planetary Science} % Meteoritics and Planetary Science
\def\nast{New Astron.}        % New Astronomy
\def\nat{Nature}              % Nature
\def\pasj{PASJ}               % Publ. of the Astronomical Society of Japan
\def\pasp{PASP}               % Publ. of the Astron. Society of the Pacific
\def\phr{Phys.~Rev.}          % Physical Review
\def\pdra{Phys.~Rev.~A}       % Physical Review A
\def\prb{Phys.~Rev.~B}       % Physical Review B
\def\prc{Phys.~Rev.~C}       % Physical Review C
\def\prd{Phys.~Rev.~D}       % Physical Review D
\def\phrep{Phys.~Rep.}        % Physics Reports
\def\phss{Phys.~Stat.~Sol.}        %
\def\procspie{Proc.~SPIE}     % Proceedings of the SPIE
\def\planss{Planet.~Space Sci.}  % Planetary & Space Sciences
\def\qjras{QJRAS}             % Quarterly Journal of the RAS
\def\rpph{Rep.~Prog.~Phys.}   % Reports on Progress in Physics
\def\rgsp{Rev.~Geophys.~Space Phys.~} % Reviews on Geophysics and Space Physics
\def\sal{Soviet Astron.~Lett.}% Soviet Astronomy Letters
\def\sci{Science}             % Science
\def\solph{Sol.~Phys.}        % Solar Physics
\def\ssr{Space Sci.~Rev.}     % Space Science Reviews
\def\zap{Z.~Astrophys.}       % Zeitschrift fuer Astrophysik

